On the Parameterized Complexity Of Grid Contraction

For a family of graphs $\mathcal{G}$, the $\mathcal{G}$-\textsc{Contraction} problem takes as an input a graph $G$ and an integer $k$, and the goal is to decide if there exists $F \subseteq E(G)$ of size at most $k$ such that $G/F$ belongs to $\mathcal{G}$. Here, $G/F$ is the graph obtained from $G$ by contracting all the edges in $F$. In this article, we initiate the study of \textsc{Grid Contraction} from the parameterized complexity point of view. We present a fixed parameter tractable algorithm, running in time $c^k \cdot |V(G)|^{\mathcal{O}(1)}$, for this problem. We complement this result by proving that unless \ETH\ fails, there is no algorithm for \textsc{Grid Contraction} with running time $c^{o(k)} \cdot |V(G)|^{\mathcal{O}(1)}$. We also present a polynomial kernel for this problem.

==> fpt-path.tex <==
\section{An \FPT\ Algorithm for \textsc{Path Contraction}}

In this section, we present an \FPT\ algorithm for \textsc{Path Contraction}. Our algorithm is inspired by the exact exponential algorithm for \textsc{Ex-Path Contraction} presented in \cite{path-contraction}. In \textsc{Ex-Path Contraction} problem, an input is a graph and the question is what is the largest integer $q$ such that the given graph can be contracted to $P_q$. We build upon the ideas presented in Section~$4.1$ in \cite{path-contraction} to solve a special case of \textsc{Ex-Path Contraction}. The idea is to build a \emph{special partial solution} for some \emph{nice subsets} of given graph. In this partial solution, all boundary vertices of a particular nice subset are contained in last bag. This partial solution is then extended to remaining graph.
The central idea in their argument is: \emph{for a nice subset $S$ of graph $G$, if $G[S]$ can be contracted to a path such that all boundary vertices of $S$ are in an end bag then how one actually contract $G[S]$ is irrelevant}.
This allows them to store one solution for $G[S]$ and build dynamic programming table.
A naive analysis of such dynamic programming procedure shows that overall running time of the algorithm is $\calO(3^n)$. 
The authors demonstrate that running time of the algorithm is $\calO((2 - \epsilon)^n)$ for some $\epsilon > 0$ by carefully bounding following two quantities $(i)$
the number of possible entries in the dynamic programming table; and $(ii)$ time spent at each entry.
% In \cite{path-contraction}, authors managed to bound the running time of the algorithm by carefully considering subsets whose closed neighborhood is at most some fixed fraction of the total number of vertices in the graph.
The authors used notation of \emph{$(a,b)$-connected subsets} to obtain the improved bound.  
They argue that to bound both these quantities it is sufficient to know the size of neighborhood of $S$ and size of $S$.
We prove that \emph{to bound both these quantities as a function of $k$, it is sufficient to know the size of neighborhood of $S$ and size of last witness set in path contraction of $G[S]$ which contains all boundary vertices of $S$}.

%This also allows them to restrict the possible expansion of partial solution for $S$. 
%\begin{definition}[Potential Witness Set]\label{def:pws} A subset $W$ of $V(G)$ is said to be a \emph{potential witness set} of $G$ if there exists a path witness structure, say $\calW$, of $G$ such that $W$ is one of the witness sets in $\calW$.  
%\end{definition}
% \begin{definition}[$k$-Potential Witness Set]\label{def:k-pws} A subset $W$ of $V(G)$ is said to be a $k$-\emph{potential witness set} of $G$ if there exists a $k$-path witness structure, say $\calW$, of $G$ such that $W$ is one of the witness sets in $\calW$. \end{definition}

For a given graph $G$ and an integer $k$, we define following terms which are used in remaining section. 
\begin{definition}[$k$-Potential Witness Set]\label{def:k-pws} A connected subset $W$ of $V(G)$ is said to be a $k$-\emph{potential witness set} of $G$ if it satisfy following two conditions:
  \begin{itemize}
  \item $|W| + |N(W)| \le k + 3$; and
  \item $G - W$ has at most two connected components.
  \end{itemize}
\end{definition}
% We note that prefix $k$ in $k$-potential witness set corresponds with number of edges we are allowed to contract in given graph to obtain a path.
We say a path witness structure of $G$ is a \emph{$k$-path witness structure} if the size of union of spanning trees of all witness sets in $\calW$ is at most $k$. The two properties mentioned in the definition of $k$-potential witness sets are result of structural properties of witness sets in $k$-path witness structure.
We note that $W = \emptyset$ is a $k$-potential witness set.
\iffalse
In the following claim, we justify that all ``potential witness structure'' have been \emph{considered} by $k$-potential witness sets.
\begin{claim} For a given graph $G$, if a subset $W$ of $V(G)$ is contained in some $k$-path witness structure of $G$ then $W$ is a $k$-potential witness set of $G$.
\end{claim}
\begin{proof} To prove that $W$ is a $k$-potential witness set, we need to argue that $|W| + |N(W)| \le k + 3$ and $G - W$ has at most two connected components.
Let $\calW = \{W_1, W_2, \dots, W_q\}$ be a $k$-path witness structure of $G$ which contains $W$. Let $W = W_i$ for some $i$ in $[q]$. Since $\calW$ is a path witness structure of $G$, witness sets $W_{i - 1}$ and $W_{i + 1}$ are adjacent with $W_i = W$. Note that one or both of them may not exists. Since we will be using upper bound on their cardinalities, this does not change the remaining argument. Let $k_{i - 1}, k_i, k_{i + 1}$ be the number of vertices in $W_{i - 1}, W_i$, and $W_{i+1}$ respectively. Since $\calW$ is a $k$-path witness structure, $(k_{i-1} - 1) + (k_i - 1) + (k_{i + 1} - 1) \le k$. By definition of contractible graphs and witness structure, all neighbors of $W$ are contained in $W_1 \cup W_2$. This implies $|W| + |N(W)| \le k + 3$. Since $\calW$ is a path-witness structure of $G$, both sets $W_1 \cup W_2 \cup \dots \cup W_{i-1}$ and $W_{i+1} \cup W_{i+2} \cup \dots W_q$ are connected subsets of $G$. Hence $G - S$ has at most two connected components. This implies that $W$ is a $k$-potential witness set of $G$.
\end{proof}
\fi
Following lemma states that for a given graph $G$, we can compute all of its $k$-potential witness sets.

\begin{lemma}\label{lemma:all-k-pws} For a graph $G$ and integer $k$ the number of $k$-potential witness sets is most $2^{k} \cdot n^{\calO(1)}$. Moreover, we can enumerate all $k$-potential witness sets in $2^{k} \cdot n^{\calO(1)}$ time.
\end{lemma}
\begin{proof}
By Corollary~\ref{cor:nr-conn-comps}, we can compute all connected sets which satisfy first property mentioned in Definition~\ref{def:k-pws}. It is polynomial time to process to check second property mentioned in Definition~\ref{def:k-pws}. The upper bound on $k$-potential witness set and running time to compute those follows from Corollary~\ref{cor:nr-conn-comps}.
\end{proof}


We use notation of $k$-potential witness sets to define \emph{nice set} mentioned in the first paragraph of this section. 
\begin{definition}[$k$-Nice-Subset]\label{def:nice-subset} A subset $S$ of $V(G)$ is said to be a $k$-\emph{nice subset} of $G$ if there exists a subset $W$ of $S$ such that $W$ is a $k$-potential witness set of $G$ and $G[S \setminus W]$ is one of the connected components of $G - W$. 
\end{definition}
\begin{figure}[t]
  \begin{center}
    \includegraphics[scale=0.05]{./images/nice-subsets.jpg}
  \end{center}
  \caption{Top Figure : Set $W$ is a $k$-potential witness set and $S = C_1 \cup W$ is a $k$-nice subset. See Defintion~\ref{def:nice-subset}. Bottom Figure : Set $A$ is a possible extention of $k$-nice subset $S$. In other words, $A$ is an element in $\calA_{|A|, |B|}[(S, x)]$. See paragraph before Lemma~\ref{lemma:algorithm-correct}. \label{fig:nice-subset}}
\end{figure}
In other words, let $W$ is a $k$-potential witness set of $G$ and $C$ be one of the connected components of $G - W$ then set $W \cup C$ is called as $k$-nice subset of $G$. See Figure~\ref{fig:nice-subset}.
We slight abuse of notation, if $G - W$ has exactly one connected component then we treat $W$ has $k$-nice subset.
As $W = \emptyset$ is a $k$-potential witness set, $V(G)$ is a $k$-nice subset.  
If $S$ is a $k$-nice subset then $G[S]$ is connected. We say a $k$-potential witness set $W$ is \emph{responsible} for $k$-nice subset $S$ if $W$ is contained in $S$ and $G[S\setminus W]$ is one of the connected components of $G - W$. Once again, with slight abuse of notation, if $G - W$ is a connected graph, we say $W$ is $k$-potential witness set which is responsible for itself.
Note that there may be more than one $k$-potential witness sets responsible for a $k$-nice subset. Let $\calS_k$ be set of all $k$-nice subsets of $G$. For every set in $\calS_k$, we associate an integer which corresponds to the size of $k$-potential witness set responsible for it.
\begin{definition}[Valid Tuple] For a set $S$ in $\calS_k$ and an integer $x$ in $[k]$, tuple $(S, x)$ is said to be a \emph{valid tuple} if there exists a $k$-potential witness set of size $x$ which is responsible for $S$. 
\end{definition}
\begin{remark}\label{remark:possible-end-bag} For a valid tuple $(S, x)$, $G - S$ is connected if and only if $|S| = x$.
\end{remark}
We note that $x \le |S|$. Let $\calV_k$ be the set of all valid tuples. Following lemma states that we can compute all valid tuple in \FPT\ time.
\begin{lemma}\label{lemma:all-k-valid-tuples} For a graph $G$ and integer $k$, the number of valid tuples is most $2^{k} \cdot n^{\calO(1)}$. Moreover, we can enumerate all valid tuples in $2^{k} \cdot n^{\calO(1)}$ time.
\end{lemma}
\begin{proof}
  By definition, if $W$ is a $k$-potential witness set then $G - W$ has at most two connected components. Hence any $k$-potential witness is responsible for at most two $k$-nice sets.
If $G - W$ has exactly one connected component, say $C_1$, we add $(V(C_1) \cup W, |W|)$ and $(W, |W|)$ to set of valid tuples. Consider the case when $G - W$ has two connected components, say $C_1, C_2$. We add $(V(C_1) \cup W, |W|)$ and $(V(C_2) \cup W, |W|)$ to set of valid tuples. By definition of $k$-nice subsets, for any $k$-nice subset there exists a $k$-potential witness set responsible for it. Hence we have constructed set of all valid tuples. The running time and upper bound on number of valid tuples follows from Lemma~\ref{lemma:all-k-pws}.
\end{proof}

We now present an overview of the algorithm. Recall that for a given connected subset $S$ of $V(G)$, $\Phi(S)$ denotes its boundary vertices i.e. set of vertices in $S$ which are adjacent with at least one vertex outside $S$.
The algorithm constructs a table in which there is an entry corresponding to every index $((S, x); k')$ where $(S, x)$ is a valid tuple in $\calV_k$ and $k'$ is an integer in $\{0\} \cup [k]$. It initialize values corresponding to all entries to \false.
From Lemma~\ref{lemma:all-k-valid-tuples}, there are at most $2^k \cdot n^{\calO(1)}$ entries in the dynamic programming table and table can be initialized in the same time.
The algorithm assign $\Gamma[(S, x); k'] = $ \true\ if $k' + |N(S)| -1 \le k$ and $G[S]$ can be $k'$-contracted to a path with all vertices in $\Phi(S)$ in the end bag of size $x$. Formally, $\Gamma[(S, x); k'] = $ \true\ if and only if $k' + |N(S)| -1 \le k$ and there is a $P_{q}$-witness structure $\{W_1,W_2,\dots, W_{q}\}$ of $G[S]$ for some integer $q$, such that $\Phi(S) \subseteq W_{q}$ and $|W_{q}| = x$. 

We slightly modify notations used in \cite{path-contraction} to explain the algorithm. For a valid tuple $(S, x)$ in $\calV_k$, let $\calA[(S, x)]$ be the set of all ``potential extenders bags'' for $S$, when we look at contraction to paths for larger graphs (containing $S$). For the sake of improved analysis, we will define $\calA_{a,b}[(S, x)] \subseteq \calA[S]$, where the sets in $\calA_{a,b}[(S, x)]$ will be of size exactly $a$ and will have exactly $b$ neighbors outside $S$ and $a + b + x \le k + 3$. Formally, $\calA_{a, b}[(S, x)] = \{A\subseteq V(G) \setminus S \mid G[A] \mbox{ is connected, } N(S) \subseteq A, |A| = a, |N(A) \setminus S| = b \mbox{ and } a + b + x \le k + 3\}$. See Figure~\ref{fig:nice-subset}.

We now describe how the algorithm computes a value for $\Gamma[(S, x); k']$ for every tuple $(S, x)$ in $\calV_k$ and every integer $k'$ in $\{0\} \cup [k]$.
As mentioned earlier, all the values in the table are initialized to \false.
The algorithm process indices in the table in chronologically increasing order. It first checks the size of $S$, then value of $x$, followed by $k$. Ties are broken arbitrarily.
For $(S, x)$ in $\calV_{k}$ such that $|S| = 1$, the algorithm sets $\Gamma[(S, 1); 0]$ to \true.
At table index $((S, x); k)$, if $\Gamma[(S, x); k]$ is \true\ then algorithm does the following: for every pair of integer $a, b$, such that $a + b + x \leq k + 3$ and $|N(S)| = y \leq a$, it computes the set $\calA_{a, b}[(S, x)]$.
%Note that $\calA_{a, b}[(S, x)]$ CAN BE COMPUTED IN time $2^{a + b - y} \cdot n^{\calO(1)}$, using Lemma~\ref{lemma:main-nr-conn-comps}.
For every set $A$ in $\calA_{a, b}[(S, x)]$, the algorithm sets $\Gamma[(S \cup A, a); k_1]$ to \true\ for every $k_1 \ge k' + (a - 1)$.
We note that once algorithm sets a particular value to \true, it does not change the value afterwords.
Intuitively speaking, $A$ is the ``new'' witness set to be ``appended'' to the witness structure of $G[S]$, to obtain a witness structure for $G[S\cup A]$. Hence if $G[S]$ can be $k'$-contracted to a path then $G[S \cup A]$ can be $k' + (|A| - 1)$-contracted to a path. We formalize this intuitation in the follwoing lemma.

\begin{algorithm}[t]
  \KwIn{A graph $G$ on $n$ vertices and an integer $k$.}
  \KwOut{\true\ if $G$ can be $k$-contracted to a path otherwise \false.}
  Compute set of valid tuples $\calV_{k}$ using Lemma~\ref{lemma:all-k-valid-tuples} \label{step:start-enitialize}\; 
  \For{$(S, x) \in \calV_{k}$, and integer $k'$ in $\{0\} \cup [k]$}{
    Initialize $\Gamma[(S, x); k'] = \false$\;
  }
  \tcc{$\Gamma[(S, x); k'] = \true$ if $k' + |N(S)| - 1 \le k$ and $G[S]$ can be $k'$-contracted to a path with all vertices in $\Phi(S)$ in the end bag of size $x$.}
  
  \For{$(S, x) \in \calV_{k}$ such that $|S| = x$ and $k' \ge |S| - 1$ \label{step:base-case}}{
    $\Gamma[(S, x); k'] = \true$\;
  }\label{step:end-initialize}

  \For{every tuple $((S, x); k')$ (in chronologically increasing order)\label{step:for-loop}}{
    \If{$\Gamma[(S, x); k']$ is $\false$}{
      Continue to next tuple in the table.
    }

    \For{every pair $(a > 0, b \ge 0)$ of integers such that $(1)\ x + a + b \le k + 3$, $(2)\ k' + a - 1 \le k$, and $(3)\ |N(S)| \leq a$}{
      
      Compute $\calA_{a, b}[(S, x)] = \{A \subseteq V(G) \setminus S \mid G[A] - S \mbox{ is connected, } N(S)\subseteq A, |A| = a, \mbox{ and } |N_{G}(A) \setminus S| = b\}$, using Lemma~\ref{lemma:main-nr-conn-comps}\;

      \For{$A \in \calA_{a, b}[(S, x)]$ and $k_1 \ge k' + a - 1 $\label{step:recurrence}}{
        $\Gamma[(S \cup A, a); k_1] = \true$ (if $k_1 + |N(S \cup A)| - 1 \le k$)\;
      }
    }
  }

  \If{ $\Gamma[(V(G), x); k']$ is set to \true\ for some values of $x$ and $k'$}{
    \Return \true\;
  }
  \Return \false\;
  \caption{\FPT\ Algorithm for \textsc{Path Contraction}  \label{algo:fpt-path-contraction}}
\end{algorithm}

\begin{lemma}\label{lemma:algorithm-correct} For every valid tuple in $(S, x)$ in $\calV_k$ and integer $k'$ in $\{0\} \cup [k]$, Algorithm~\ref{algo:fpt-path-contraction} correctly computes $\Gamma[(S, x); k']$.
\end{lemma}
\begin{proof} We consider two cases based on cardinality of $S$ and $x$. If $x = |S|$ then by Remark~\ref{remark:possible-end-bag}, $G - S$ is connected. Any connected subset of graph can be contracted to a vertex by contracting a spanning tree. Hence the values assigned by the algorithm in \emph{for}-loop starting at Step~\ref{step:base-case} are correct.
  Note that these values are not modified at any other step in the algorithm (as $a$ is non-zero).
  In the remaining proof,  we consider indices for which $x < |S|$.

We prove the lemma by induction on $|S| + k'$ for indices $((S, x); k')$ in the dynamic programming table.
For the induction hypothesis, we assume that for a positive integer $r$ the algorithm computes $\Gamma[(S, x); k']$ correctly for each $(S, x)$ in $\calV_k$ and $k'$ in $0 \cup [k]$ for which $|S| + k' \leq r$.
Consider the base case when $|S| = 1$ and $k' = 0$. As mentioned in previous paragraph, the algorithm correctly computes $\Gamma[(S, 1); 0]$ for all $(S, x)$ in $\calV_k$ for which $|S| = 1$.
%Since any vertex is a path, the values assigned by the algorithm in \emph{for}-loop starting at Step~\ref{step:base-case} are correct.
% Thus, the algorithm correctly computes $\Gamma[(S, x); 0]$ for all $(S, x)$ in $\calV_k$ for which $|S| = 1$.
Assuming induction hypothesis, we now argue that the computation of $\Gamma[\cdot]$ for indices of the form $((S_1, x_1), k_1)$ where $|S_1| + k_1 = r + 1$ are correct.
  % Consider an index $((S_1, x_1); k_1)$ in dynamic programming table such that $|S_1| + k_1 = r + 1$.
  As $((S_1, x_1); k_1)$ is an entry in the table, $(S_1, x_1)$ is a valid tuple in $\calV_k$ and $k_1$ is in $\{0\} \cup [k]$.

  Assume that $G[S_1]$ is $k_1$-contractible to a path such that all vertices in $\Phi(S_1)$ are in an end bag of size $x_1$ and $k_1 + |N(S_1)| - 1 \le k$. We argue that the algorithm sets $\Gamma[(S_1, x_1); k_1]$ to \true.
  Let $G[S_1]$ be $k_1$-contractible to path $P_q$. If $q = 1$ then, by Remark~\ref{remark:possible-end-bag}, $x_1 = |S_1|$. As discussed in first paragraph, in this case algorithm correctly computes $\Gamma[(S_1, x_1), k_1]$. Consider the case when $q \ge 2$. Let $\calW = \{W_1, \dots,  W_{q - 1}, W_q\}$ be a $P_q$-witness structure of $G[S_1]$ such that $\Phi(S_1) \subseteq W_q $ and $|W_q| = x_1$. Consider set $S_0 = W_1 \cup W_2 \cup \cdots \cup W_{q - 1}$. Since $q \ge 2$, $S_0$ is an non-empty set. Let $|W_{q - 1}| = x_0$ and $k_0 = k_1 - (|W_{q - 1}| - 1)$. We argue that $((S_0,x_0); k_0)$ is an index in the table and $|S_0| + k_0 \le r$. As $\calW$ is a $k_1$-path witness structure, $|W_{q - 1}| - 1 \le k_1$ and hence $k_0$ is an non-negative integer. Note that $G[W_q]$ is a connected graph and every connected component of $G - W_q$ is adjacent with $W_q$. Hence $G - W_{q-1}$ has exactly two connected components viz $G[W_1\cup \cdots W_{q-2}]$ and the component containing $W_q$. Moreover, as $\calW$ is a $k_1$-path witness structure, $|W_{q - 2}| + |W_{q - 1}| + |W_q| \le k_1 + 3 \le k + 3$ and $N(W_q) \subseteq W_{q - 2} \cup W_{q}$. (We note that $W_{q -2}$ may not exists but this does not change the argument. For the sake of clarity, we do not consider this as separate case.) Since $|W_{q-1}| + |N(W_{q-1})| \le k + 3$ and $G - W_{q-1}$ has at most two connected components, $W_{q - 1}$ is a $k$-potential witness set. Hence $(S_0, |W_{q -1}| = x_0)$ is a tuple in $\calV_k$ and $((S_0, x_0); k_0)$ is an index in the table. Since $W_q$ is not an empty set, $|S_0| + k_0 \le |S_1| - |W_q| + k_1 - (|W_q| - 1) \le r + 2(1 - |W_q|) \le r$. Note that $\calW \setminus \{W_q\}$ is a $(k_1 - |W_q| + 1)$-path witness structure for $G[S_0]$ which implies that $G[S_0]$ is $k_0$-path contractible with $\Phi(S_0)$ in an end bag of size $x_0$ and $k_0 + |N(S_0)| - 1 \le k_1 \le k$. 
  By the induction hypothesis, the algorithm has correctly set $\Gamma[(S_0, x_0); k_0]$ to \true.
Let $a = |W_q|$ and $b = |W_q \setminus N(S_0)| = |N(S_1)| $. We first claim that $x_0 + a + b \le k + 3$. Note that $|W_{q - 1}| + |W_q| \le k_1 + 2$ and $k_1 + b \le k + 1$. Hence $|W_{q - 1}| + |W_q| + b = x_0 + a + b \le k + 3$. 
At index $((S_0, x_0); k_0)$, the algorithm computes $\calA_{a,b}[(S_0, x_0)]$. Clearly, $W_q$ is one of the sets in $\calA_{a,b}[(S_0, x_0)]$. Hence the algorithm sets $\Gamma[(S_1, x_1), k_1]$ to \true.

To prove other direction, we assume that the algorithm sets $\Gamma[(S_1, x_1); k_1]$ to $\true$. We argue that $G[S_1]$ is $k_1$-contractible to a path such that all vertices in $\Phi(S_1)$ are in an end bag of size $x_1$ and $k_1 + |N(S_1)| - 1 \le k$. If 
$\Gamma[(S_1, x_1); k_1]$ is set to $\true$ in the \emph{for}-loop started at Step~\ref{step:base-case}, then, as discussed in first paragraph, this is correct. We now consider the case when value at $\Gamma[(S_1, x_1); k_1]$ is changed while algorithm was processing at index $((S_0, x_0); k_0)$ which has been set \true\ by the algorithm.
Let $A$ be the set in $\calA_{a, b}[(S_0, x_0)]$ such that $S_1 = S_0 \cup A$ where $a = |A|$ and $b = |N(S_1)|$. Since $a$ is a positive integer and $k_0 + a - 1 \le k_1$, we know $|S_0| + k_0 \le |S_1| + k_1 - 2a + 1 = r - 2a + 1$. By the induction hypothesis, algorithm correctly computes value at $((S_0, x_0); k_0)$. Hence $G[S_0]$ can be $k_0$-contracted to a path with all vertices in $\Phi(S_0)$ in one of end bag of size $x_0$ and $k_0 + |N(S_0)| - 1 \le k + 3$. As the algorithm computes connected set $A$ in $V(G) \setminus S_1$ such that $N(S_0) \subseteq A$, $G[S_1]$ can be $k_1$-contracted to a path with all vertices in $\Phi(S)$ in an end bag (which is $A$) of size $x_1 = a$. It remains to argue that $k_1 + |N(S_1)| - 1 \le k$.
We prove this for the case $k_1 = k_0 + a - 1$ as $k_1 > k_0 + a - 1$ case follows from the definition of $k_1$-contratibility. As $x_0$ is the size of an end back, $x_0 - 1 \le k_0$. As algorithm only considers $a, b$ such that $x_0 + a + b \le k + 3$, substituting $a = k_1 - k_0 + 1$ and $b = |N(S_1)|$ we get $x_0 + k_1 - k_0 + 1 + |N(S_1)| \le k + 3$. Using $x_0 - 1 \le k$, we get desired bound. This completes the proof of the lemma.  
\end{proof}

We are now in a position to present main result of this section.
\begin{theorem}\label{lem:correct-runtime-EPPC}
  \sloppy \textsc{Path Contraction} admits an algorithm with running time $2^{k} \cdot n^{\calO(1)}$. Here, $n$ is the number of vertices in input graph. 
\end{theorem}
\begin{proof} The correctness of the algorithm follows from the fact that $(V(G), x)$ is a tuple in $\calV_k$ for some $x$ and Lemma~\ref{lemma:algorithm-correct}. By Lemma~\ref{lemma:all-k-valid-tuples}, Step \ref{step:start-enitialize}-\ref{step:end-initialize} of the algorithm can be executed in time $2^k \cdot n^{\calO(1)}$. We argue that the \emph{for}-loop starting at Step~\ref{step:for-loop} takes $2^k \cdot n^{\calO(1)}$ time to complete. We partition set of valid tuples $\calV_k$ using the sizes of neighborhood of set in tuple, and an integer at second place in tuple. For two fixed integers $x, y$, define $\calV_k^{x, y} := \{(S, x') \in \calV_k |\ x' = x \text{ and } |N(S)| = y \}$. In other words, $\calV_k^{x, y}$ collection of all $k$-nice subsets (and an associated integer) whose neighborhood is of size $y$ and there is a $k$-potential witness set of size $x$ responsible for it. Alternatively, $\calV_k^{x, y}$ is collection of $k$-nice subsets for which there is a $(x, y)$-connected $k$-potential witness set which is responsible for it. Since the number of $(x, y)$-connected subsets are bounded (Corollary~\ref{cor:nr-conn-comps}) and each $k$-potential witness set is responsible for at most two $k$-nice subsets, $|\calV_k^{x,y}|$ is bounded by $2^{x+y} \cdot n^{\calO(1)}$.

  For each $ (S, x) \in \calV_k^{x,y}$, the algorithm considers every pair of integers $a (> 0), b (\ge 0)$, such that $x + a + b \leq k + 3$ and $ |N(S)| = y \leq a$, and computes the set $\calA_{a, b}[(S, x)]$. By Lemma \ref{lemma:main-nr-conn-comps}, set $\calA_{a, b}[(S, x)]$ can be computed in time $2^{a+b-|N(S)|} \cdot n^{\calO(1)}$. 
  The algorithm spends time proportional to $|\calA_{a, b}[(S, x)]|$ for \emph{for}-loop starting at Step~\ref{step:recurrence}. Hence for two fixed integers $x, y$, algorithm spends 
$$
\sum_{\substack{a,b \\ x+a+b \leq k + 3}} 
 2^{x+y} \cdot 2^{a+b-y} \cdot n^{\calO(1)} =  
\sum_{\substack{a,b \\ x+a+b \leq k + 3}} 
 2^{x+a+b} 
 \cdot n^{\calO(1)} = 2^k \cdot n^{\calO(1)}
 $$
time to process all valid tuples in $\calV_k^{x, y}$. Since there are at most $\calO(k^2)$ feasible values for $x, y$, the overall running time of algorithm is bounded by $2^k \cdot n^{\calO(1)}$.
 This concludes the proof.
\end{proof}


==> fpt.tex <==
\section{\FPT\ Algorithm for \textsc{Path Contraction}}

In this section, we present an \FPT\ algorithm for \textsc{Path Contraction}. Our algorithm is inspired by the exact exponential algorithm for \textsc{Ex-Path Contraction} presented in \cite{path-contraction}. In \textsc{Ex-Path Contraction} problem, an input is a graph and the question is what is the largest integer $q$ such that the given graph can be contracted to $P_q$. We build upon the ideas presented in Section~$4.1$ in \cite{path-contraction} to solve a special case of \textsc{Ex-Path Contraction}. The idea is to build a \textsc{special partial solution} for some \emph{nice subsets} of given graph. In this partial solution, all boundary vertices of a particular nice subset are contained in last bag. This partial solution is then extended to remaining graph.
The central idea in their argument is: \emph{for a nice subset $S$ of graph $G$, if $G[S]$ can be contracted to a path such that all boundary vertices of $S$ are in an end bag then how one actually contract $G[S]$ is irrelevant}.
This allows them to store one solution for $G[S]$ and build dynamic programming table.
The trivial analysis of such dynamic programming procedure shows that overall running time of the algorithm is $\calO(3^n)$. 
The authors demonstrate that running time of the algorithm is $\calO((2 - \epsilon)^n)$ for some $\epsilon > 0$ by carefully bounding following two quantities $(i)$
the number of possible entries in the dynamic programming table; and $(ii)$ time spent at each entry.
% In \cite{path-contraction}, authors managed to bound the running time of the algorithm by carefully considering subsets whose closed neighborhood is at most some fixed fraction of the total number of vertices in the graph.
The authors used notation of \emph{$(a,b)$-connected subsets} to obtain the improved bound.  
The authors argue that to bound both these quantities it is sufficient to know the size of neighborhood of $S$ and size of $S$.
We prove that \emph{to bound both these quantities as a function of $k$, it is sufficient to know the size of neighborhood of $S$ and size of last witness set in path contraction of $G[S]$ which contains all boundary vertices of $S$}.

%This also allows them to restrict the possible expansion of partial solution for $S$. 
%\begin{definition}[Potential Witness Set]\label{def:pws} A subset $W$ of $V(G)$ is said to be a \emph{potential witness set} of $G$ if there exists a path witness structure, say $\calW$, of $G$ such that $W$ is one of the witness sets in $\calW$.  
%\end{definition}
% \begin{definition}[$k$-Potential Witness Set]\label{def:k-pws} A subset $W$ of $V(G)$ is said to be a $k$-\emph{potential witness set} of $G$ if there exists a $k$-path witness structure, say $\calW$, of $G$ such that $W$ is one of the witness sets in $\calW$. \end{definition}

For a given graph $G$ and an integer $k$, we define following terms which are used in remaining section. 
\begin{definition}[$k$-Potential Witness Set]\label{def:k-pws} A connected subset $W$ of $V(G)$ is said to be a $k$-\emph{potential witness set} of $G$ if it satisfy following two conditions:
  \begin{itemize}
  \item $|W| + |N(W)| \le k + 3$; and
  \item $G - W$ has at most two connected components.
  \end{itemize}
\end{definition}
% We note that prefix $k$ in $k$-potential witness set corresponds with number of edges we are allowed to contract in given graph to obtain a path.
We say a path witness structure of $G$ is a \emph{$k$-path witness structure} if the size of union of spanning trees of all witness sets in $\calW$ is at most $k$. The two properties mentioned in the definition of $k$-potential witness sets are result of structural properties of witness sets in $k$-path witness structure.
We note that $W = \emptyset$ is a $k$-potential witness set.
\iffalse
In the following claim, we justify that all ``potential witness structure'' have been \emph{considered} by $k$-potential witness sets.
\begin{claim} For a given graph $G$, if a subset $W$ of $V(G)$ is contained in some $k$-path witness structure of $G$ then $W$ is a $k$-potential witness set of $G$.
\end{claim}
\begin{proof} To prove that $W$ is a $k$-potential witness set, we need to argue that $|W| + |N(W)| \le k + 3$ and $G - W$ has at most two connected components.
Let $\calW = \{W_1, W_2, \dots, W_q\}$ be a $k$-path witness structure of $G$ which contains $W$. Let $W = W_i$ for some $i$ in $[q]$. Since $\calW$ is a path witness structure of $G$, witness sets $W_{i - 1}$ and $W_{i + 1}$ are adjacent with $W_i = W$. Note that one or both of them may not exists. Since we will be using upper bound on their cardinalities, this does not change the remaining argument. Let $k_{i - 1}, k_i, k_{i + 1}$ be the number of vertices in $W_{i - 1}, W_i$, and $W_{i+1}$ respectively. Since $\calW$ is a $k$-path witness structure, $(k_{i-1} - 1) + (k_i - 1) + (k_{i + 1} - 1) \le k$. By definition of contractible graphs and witness structure, all neighbors of $W$ are contained in $W_1 \cup W_2$. This implies $|W| + |N(W)| \le k + 3$. Since $\calW$ is a path-witness structure of $G$, both sets $W_1 \cup W_2 \cup \dots \cup W_{i-1}$ and $W_{i+1} \cup W_{i+2} \cup \dots W_q$ are connected subsets of $G$. Hence $G - S$ has at most two connected components. This implies that $W$ is a $k$-potential witness set of $G$.
\end{proof}
\fi
Following lemma states that for a given graph $G$, we can compute all of its $k$-potential witness sets.

\begin{lemma}\label{lemma:all-k-pws} For a graph $G$ and integer $k$ the number of $k$-potential witness sets is most $2^{k} \cdot n^{\calO(1)}$. Moreover, we can enumerate all $k$-potential witness sets in $2^{k} \cdot n^{\calO(1)}$ time.
\end{lemma}
\begin{proof}
By Corollary~\ref{cor:nr-conn-comps}, we can compute all connected sets which satisfy first property mentioned in Definition~\ref{def:k-pws}. It is polynomial time to process to check second property mentioned in Definition~\ref{def:k-pws}. The upper bound on $k$-potential witness set and running time to compute those follows from Corollary~\ref{cor:nr-conn-comps}.
\end{proof}


We use notation of $k$-potential witness sets to define \emph{nice set} mentioned in the first paragraph of this section. 
\begin{definition}[$k$-Nice-Subset]\label{def:nice-subset} A subset $S$ of $V(G)$ is said to be a $k$-\emph{nice subset} of $G$ if there exists a subset $W$ of $S$ such that $W$ is a $k$-potential witness set of $G$ and $G[S \setminus W]$ is one of the connected components of $G - W$. 
\end{definition}
\begin{figure}[t]
  \begin{center}
    \includegraphics[scale=0.05]{./images/nice-subsets.jpg}
  \end{center}
  \caption{Top Figure : Set $W$ is a $k$-potential witness set and $S = C_1 \cup W$ is a $k$-nice subset. See Defintion~\ref{def:nice-subset}. Bottom Figure : Set $A$ is a possible extention of $k$-nice subset $S$. In other words, $A$ is an element in $\calA_{|A|, |B|}[(S, x)]$. See paragraph before Lemma~\ref{lemma:algorithm-correct}. \label{fig:nice-subset}}
\end{figure}
In other words, let $W$ is a $k$-potential witness set of $G$ and $C$ be one of the connected components of $G - W$ then set $W \cup C$ is called as $k$-nice subset of $G$. See Figure~\ref{fig:nice-subset}.
We slight abuse of notation, if $G - W$ has exactly one connected component then we treat $W$ has $k$-nice subset.
As $W = \emptyset$ is a $k$-potential witness set, $V(G)$ is a $k$-nice subset.  
If $S$ is a $k$-nice subset then $G[S]$ is connected. We say a $k$-potential witness set $W$ is \emph{responsible} for $k$-nice subset $S$ if $W$ is contained in $S$ and $G[S\setminus W]$ is one of the connected components of $G - W$. Once again, with slight abuse of notation, if $G - W$ is a connected graph, we say $W$ is $k$-potential witness set which is responsible for itself.
Note that there may be more than one $k$-potential witness sets responsible for a $k$-nice subset. Let $\calS_k$ be set of all $k$-nice subsets of $G$. For every set in $\calS_k$, we associate an integer which corresponds to the size of $k$-potential witness set responsible for it.
\begin{definition}[Valid Tuple] For a set $S$ in $\calS_k$ and an integer $x$ in $[k]$, tuple $(S, x)$ is said to be a \emph{valid tuple} if there exists a $k$-potential witness set of size $x$ which is responsible for $S$. 
\end{definition}
\begin{remark}\label{remark:possible-end-bag} For a valid tuple $(S, x)$, $G - S$ is connected if and only if $|S| = x$.
\end{remark}
We note that $x \le |S|$. Let $\calV_k$ be the set of all valid tuples. Following lemma states that we can compute all valid tuple in \FPT\ time.
\begin{lemma}\label{lemma:all-k-valid-tuples} For a graph $G$ and integer $k$, the number of valid tuples is most $2^{k} \cdot n^{\calO(1)}$. Moreover, we can enumerate all valid tuples in $2^{k} \cdot n^{\calO(1)}$ time.
\end{lemma}
\begin{proof}
  By definition, if $W$ is a $k$-potential witness set then $G - W$ has at most two connected components. Hence any $k$-potential witness is responsible for at most two $k$-nice sets.
If $G - W$ has exactly one connected component, say $C_1$, we add $(V(C_1) \cup W, |W|)$ and $(W, |W|)$ to set of valid tuples. Consider the case when $G - W$ has two connected components, say $C_1, C_2$. We add $(V(C_1) \cup W, |W|)$ and $(V(C_2) \cup W, |W|)$ to set of valid tuples. By definition of $k$-nice subsets, for any $k$-nice subset there exists a $k$-potential witness set responsible for it. Hence we have constructed set of all valid tuples. The running time and upper bound on number of valid tuples follows from Lemma~\ref{lemma:all-k-pws}.
\end{proof}

We now present an overview of the algorithm. Recall that for a given connected subset $S$ of $V(G)$, $\Phi(S)$ denotes its boundary vertices i.e. set of vertices in $S$ which are adjacent with at least one vertex outside $S$.
The algorithm constructs a table in which there is an entry corresponding to every index $((S, x); k')$ where $(S, x)$ is a valid tuple in $\calV_k$ and $k'$ is an integer in $\{0\} \cup [k]$. It initialize values corresponding to all entries to \false.
From Lemma~\ref{lemma:all-k-valid-tuples}, there are at most $2^k \cdot n^{\calO(1)}$ entries in the dynamic programming table and table can be initialized in the same time.
The algorithm assign $\Gamma[(S, x); k'] = $ \true\ if $k' + |N(S)| -1 \le k$ and $G[S]$ can be $k'$-contracted to a path with all vertices in $\Phi(S)$ in the end bag of size $x$. Formally, $\Gamma[(S, x); k'] = $ \true\ if and only if $k' + |N(S)| -1 \le k$ and there is a $P_{q}$-witness structure $\{W_1,W_2,\dots, W_{q}\}$ of $G[S]$ for some integer $q$, such that $\Phi(S) \subseteq W_{q}$ and $|W_{q}| = x$. 

We slightly modify notations used in \cite{path-contraction} to explain the algorithm. For a valid tuple $(S, x)$ in $\calV_k$, let $\calA[(S, x)]$ be the set of all ``potential extenders bags'' for $S$, when we look at contraction to paths for larger graphs (containing $S$). For the sake of improved analysis, we will define $\calA_{a,b}[(S, x)] \subseteq \calA[S]$, where the sets in $\calA_{a,b}[(S, x)]$ will be of size exactly $a$ and will have exactly $b$ neighbors outside $S$ and $a + b + x \le k + 3$. Formally, $\calA_{a, b}[(S, x)] = \{A\subseteq V(G) \setminus S \mid G[A] \mbox{ is connected, } N(S) \subseteq A, |A| = a, |N(A) \setminus S| = b \mbox{ and } a + b + x \le k + 3\}$. See Figure~\ref{fig:nice-subset}.

We now describe how the algorithm computes a value for $\Gamma[(S, x); k']$ for every tuple $(S, x)$ in $\calV_k$ and every integer $k'$ in $\{0\} \cup [k]$.
As mentioned earlier, all the values in the table are initialized to \false.
The algorithm process indices in the table in chronologically increasing order. It first checks the size of $S$, then value of $x$, followed by $k$. Ties are broken arbitrarily.
For $(S, x)$ in $\calV_{k}$ such that $|S| = 1$, the algorithm sets $\Gamma[(S, 1); 0]$ to \true.
At table index $((S, x); k)$, if $\Gamma[(S, x); k]$ is \true\ then algorithm does the following: for every pair of integer $a, b$, such that $a + b + x \leq k + 3$ and $|N(S)| = y \leq a$, it computes the set $\calA_{a, b}[(S, x)]$.
%Note that $\calA_{a, b}[(S, x)]$ can be computed in time $2^{a + b - y} \cdot n^{\calO(1)}$, using Lemma~\ref{lemma:main-nr-conn-comps}.
For every set $A$ in $\calA_{a, b}[(S, x)]$, the algorithm sets $\Gamma[(S \cup A, a); k_1]$ to \true\ for every $k_1 \ge k' + (a - 1)$.
We note that once algorithm sets a particular value to \true, it does not change the value afterwords.
Intuitively speaking, $A$ is the ``new'' witness set to be ``appended'' to the witness structure of $G[S]$, to obtain a witness structure for $G[S\cup A]$. Hence if $G[S]$ can be $k'$-contracted to a path then $G[S \cup A]$ can be $k' + (|A| - 1)$-contracted to a path. We formalize this intuitation in the follwoing lemma.

\begin{algorithm}[t]
  \KwIn{A graph $G$ on $n$ vertices and an integer $k$.}
  \KwOut{\true\ if $G$ can be $k$-contracted to a path otherwise \false.}
  Compute set of valid tuples $\calV_{k}$ using Lemma~\ref{lemma:all-k-valid-tuples} \label{step:start-enitialize}\; 
  \For{$(S, x) \in \calV_{k}$, and integer $k'$ in $\{0\} \cup [k]$}{
    Initialize $\Gamma[(S, x); k'] = \false$\;
  }
  \tcc{$\Gamma[(S, x); k'] = \true$ if $k' + |N(S)| - 1 \le k$ and $G[S]$ can be $k'$-contracted to a path with all vertices in $\Phi(S)$ in the end bag of size $x$.}
  
  \For{$(S, x) \in \calV_{k}$ such that $|S| = x$ and $k' \ge |S| - 1$ \label{step:base-case}}{
    $\Gamma[(S, x); k'] = \true$\;
  }\label{step:end-initialize}

  \For{every tuple $((S, x); k')$ (in chronologically increasing order)\label{step:for-loop}}{
    \If{$\Gamma[(S, x); k']$ is $\false$}{
      Continue to next tuple in the table.
    }

    \For{every pair $(a > 0, b \ge 0)$ of integers such that $(1)\ x + a + b \le k + 3$, $(2)\ k' + a - 1 \le k$, and $(3)\ |N(S)| \leq a$}{
      
      Compute $\calA_{a, b}[(S, x)] = \{A \subseteq V(G) \setminus S \mid G[A] - S \mbox{ is connected, } N(S)\subseteq A, |A| = a, \mbox{ and } |N_{G}(A) \setminus S| = b\}$, using Lemma~\ref{lemma:main-nr-conn-comps}\;

      \For{$A \in \calA_{a, b}[(S, x)]$ and $k_1 \ge k' + a - 1 $\label{step:recurrence}}{
        $\Gamma[(S \cup A, a); k_1] = \true$ (if $k_1 + |N(S \cup A)| - 1 \le k$)\;
      }
    }
  }

  \If{ $\Gamma[(V(G), x); k']$ is set to \true\ for some values of $x$ and $k'$}{
    \Return \true\;
  }
  \Return \false\;
  \caption{\FPT\ Algorithm for \textsc{Path Contraction}  \label{algo:fpt-path-contraction}}
\end{algorithm}

\begin{lemma}\label{lemma:algorithm-correct} For every valid tuple in $(S, x)$ in $\calV_k$ and integer $k'$ in $\{0\} \cup [k]$, Algorithm~\ref{algo:fpt-path-contraction} correctly computes $\Gamma[(S, x); k']$.
\end{lemma}
\begin{proof} We consider two cases based on cardinality of $S$ and $x$. If $x = |S|$ then by Remark~\ref{remark:possible-end-bag}, $G - S$ is connected. Any connected subset of graph can be contracted to a vertex by contracting a spanning tree. Hence the values assigned by the algorithm in \emph{for}-loop starting at Step~\ref{step:base-case} are correct.
  Note that these values are not modified at any other step in the algorithm (as $a$ is non-zero).
  In the remaining proof,  we consider indices for which $x < |S|$.

We prove the lemma by induction on $|S| + k'$ for indices $((S, x); k')$ in the dynamic programming table.
For the induction hypothesis, we assume that for a positive integer $r$ the algorithm computes $\Gamma[(S, x); k']$ correctly for each $(S, x)$ in $\calV_k$ and $k'$ in $0 \cup [k]$ for which $|S| + k' \leq r$.
Consider the base case when $|S| = 1$ and $k' = 0$. As mentioned in previous paragraph, the algorithm correctly computes $\Gamma[(S, 1); 0]$ for all $(S, x)$ in $\calV_k$ for which $|S| = 1$.
%Since any vertex is a path, the values assigned by the algorithm in \emph{for}-loop starting at Step~\ref{step:base-case} are correct.
% Thus, the algorithm correctly computes $\Gamma[(S, x); 0]$ for all $(S, x)$ in $\calV_k$ for which $|S| = 1$.
Assuming induction hypothesis, we now argue that the computation of $\Gamma[\cdot]$ for indices of the form $((S_1, x_1), k_1)$ where $|S_1| + k_1 = r + 1$ are correct.
  % Consider an index $((S_1, x_1); k_1)$ in dynamic programming table such that $|S_1| + k_1 = r + 1$.
  As $((S_1, x_1); k_1)$ is an entry in the table, $(S_1, x_1)$ is a valid tuple in $\calV_k$ and $k_1$ is in $\{0\} \cup [k]$.

  Assume that $G[S_1]$ is $k_1$-contractible to a path such that all vertices in $\Phi(S_1)$ are in an end bag of size $x_1$ and $k_1 + |N(S_1)| - 1 \le k$. We argue that the algorithm sets $\Gamma[(S_1, x_1); k_1]$ to \true.
  Let $G[S_1]$ be $k_1$-contractible to path $P_q$. If $q = 1$ then, by Remark~\ref{remark:possible-end-bag}, $x_1 = |S_1|$. As discussed in first paragraph, in this case algorithm correctly computes $\Gamma[(S_1, x_1), k_1]$. Consider the case when $q \ge 2$. Let $\calW = \{W_1, \dots,  W_{q - 1}, W_q\}$ be a $P_q$-witness structure of $G[S_1]$ such that $\Phi(S_1) \subseteq W_q $ and $|W_q| = x_1$. Consider set $S_0 = W_1 \cup W_2 \cup \cdots \cup W_{q - 1}$. Since $q \ge 2$, $S_0$ is an non-empty set. Let $|W_{q - 1}| = x_0$ and $k_0 = k_1 - (|W_{q - 1}| - 1)$. We argue that $((S_0,x_0); k_0)$ is an index in the table and $|S_0| + k_0 \le r$. As $\calW$ is a $k_1$-path witness structure, $|W_{q - 1}| - 1 \le k_1$ and hence $k_0$ is an non-negative integer. Note that $G[W_q]$ is a connected graph and every connected component of $G - W_q$ is adjacent with $W_q$. Hence $G - W_{q-1}$ has exactly two connected components viz $G[W_1\cup \cdots W_{q-2}]$ and the component containing $W_q$. Moreover, as $\calW$ is a $k_1$-path witness structure, $|W_{q - 2}| + |W_{q - 1}| + |W_q| \le k_1 + 3 \le k + 3$ and $N(W_q) \subseteq W_{q - 2} \cup W_{q}$. (We note that $W_{q -2}$ may not exists but this does not change the argument. For the sake of clarity, we do not consider this as separate case.) Since $|W_{q-1}| + |N(W_{q-1})| \le k + 3$ and $G - W_{q-1}$ has at most two connected components, $W_{q - 1}$ is a $k$-potential witness set. Hence $(S_0, |W_{q -1}| = x_0)$ is a tuple in $\calV_k$ and $((S_0, x_0); k_0)$ is an index in the table. Since $W_q$ is not an empty set, $|S_0| + k_0 \le |S_1| - |W_q| + k_1 - (|W_q| - 1) \le r + 2(1 - |W_q|) \le r$. Note that $\calW \setminus \{W_q\}$ is a $(k_1 - |W_q| + 1)$-path witness structure for $G[S_0]$ which implies that $G[S_0]$ is $k_0$-path contractible with $\Phi(S_0)$ in an end bag of size $x_0$ and $k_0 + |N(S_0)| - 1 \le k_1 \le k$. 
  By the induction hypothesis, the algorithm has correctly set $\Gamma[(S_0, x_0); k_0]$ to \true.
Let $a = |W_q|$ and $b = |W_q \setminus N(S_0)| = |N(S_1)| $. We first claim that $x_0 + a + b \le k + 3$. Note that $|W_{q - 1}| + |W_q| \le k_1 + 2$ and $k_1 + b \le k + 1$. Hence $|W_{q - 1}| + |W_q| + b = x_0 + a + b \le k + 3$. 
At index $((S_0, x_0); k_0)$, the algorithm computes $\calA_{a,b}[(S_0, x_0)]$. Clearly, $W_q$ is one of the sets in $\calA_{a,b}[(S_0, x_0)]$. Hence the algorithm sets $\Gamma[(S_1, x_1), k_1]$ to \true.

To prove other direction, we assume that the algorithm sets $\Gamma[(S_1, x_1); k_1]$ to $\true$. We argue that $G[S_1]$ is $k_1$-contractible to a path such that all vertices in $\Phi(S_1)$ are in an end bag of size $x_1$ and $k_1 + |N(S_1)| - 1 \le k$. If 
$\Gamma[(S_1, x_1); k_1]$ is set to $\true$ in the \emph{for}-loop started at Step~\ref{step:base-case}, then, as discussed in first paragraph, this is correct. We now consider the case when value at $\Gamma[(S_1, x_1); k_1]$ is changed while algorithm was processing at index $((S_0, x_0); k_0)$ which has been set \true\ by the algorithm.
Let $A$ be the set in $\calA_{a, b}[(S_0, x_0)]$ such that $S_1 = S_0 \cup A$ where $a = |A|$ and $b = |N(S_1)|$. Since $a$ is a positive integer and $k_0 + a - 1 \le k_1$, we know $|S_0| + k_0 \le |S_1| + k_1 - 2a + 1 = r - 2a + 1$. By the induction hypothesis, algorithm correctly computes value at $((S_0, x_0); k_0)$. Hence $G[S_0]$ can be $k_0$-contracted to a path with all vertices in $\Phi(S_0)$ in one of end bag of size $x_0$ and $k_0 + |N(S_0)| - 1 \le k + 3$. As the algorithm computes connected set $A$ in $V(G) \setminus S_1$ such that $N(S_0) \subseteq A$, $G[S_1]$ can be $k_1$-contracted to a path with all vertices in $\Phi(S)$ in an end bag (which is $A$) of size $x_1 = a$. It remains to argue that $k_1 + |N(S_1)| - 1 \le k$.
We prove this for the case $k_1 = k_0 + a - 1$ as $k_1 > k_0 + a - 1$ case follows from the definition of $k_1$-contratibility. As $x_0$ is the size of an end back, $x_0 - 1 \le k_0$. As algorithm only considers $a, b$ such that $x_0 + a + b \le k + 3$, substituting $a = k_1 - k_0 + 1$ and $b = |N(S_1)|$ we get $x_0 + k_1 - k_0 + 1 + |N(S_1)| \le k + 3$. Using $x_0 - 1 \le k$, we get desired bound. This completes the proof of the lemma.  
\end{proof}

We are now in a position to present main result of this section.
\begin{theorem}\label{lem:correct-runtime-EPPC}
  \sloppy \textsc{Path Contraction} admits an algorithm with running time $2^{k} \cdot n^{\calO(1)}$. Here, $n$ is the number of vertices in input graph. 
\end{theorem}
\begin{proof} The correctness of the algorithm follows from the fact that $(V(G), x)$ is a tuple in $\calV_k$ for some $x$ and Lemma~\ref{lemma:algorithm-correct}. By Lemma~\ref{lemma:all-k-valid-tuples}, Step \ref{step:start-enitialize}-\ref{step:end-initialize} of the algorithm can be executed in time $2^k \cdot n^{\calO(1)}$. We argue that the \emph{for}-loop starting at Step~\ref{step:for-loop} takes $2^k \cdot n^{\calO(1)}$ time to complete. We partition set of valid tuples $\calV_k$ using the sizes of neighborhood of set in tuple, and an integer at second place in tuple. For two fixed integers $x, y$, define $\calV_k^{x, y} := \{(S, x') \in \calV_k |\ x' = x \text{ and } |N(S)| = y \}$. In other words, $\calV_k^{x, y}$ collection of all $k$-nice subsets (and an associated integer) whose neighborhood is of size $y$ and there is a $k$-potential witness set of size $x$ responsible for it. Alternatively, $\calV_k^{x, y}$ is collection of $k$-nice subsets for which there is a $(x, y)$-connected $k$-potential witness set which is responsible for it. Since the number of $(x, y)$-connected subsets are bounded (Corollary~\ref{cor:nr-conn-comps}) and each $k$-potential witness set is responsible for at most two $k$-nice subsets, $|\calV_k^{x,y}|$ is bounded by $2^{x+y} \cdot n^{\calO(1)}$.

  For each $ (S, x) \in \calV_k^{x,y}$, the algorithm considers every pair of integers $a (> 0), b (\ge 0)$, such that $x + a + b \leq k + 3$ and $ |N(S)| = y \leq a$, and computes the set $\calA_{a, b}[(S, x)]$. By Lemma \ref{lemma:main-nr-conn-comps}, set $\calA_{a, b}[(S, x)]$ can be computed in time $2^{a+b-|N(S)|} \cdot n^{\calO(1)}$. 
  The algorithm spends time proportional to $|\calA_{a, b}[(S, x)]|$ for \emph{for}-loop starting at Step~\ref{step:recurrence}. Hence for two fixed integers $x, y$, algorithm spends 
$$
\sum_{\substack{a,b \\ x+a+b \leq k + 3}} 
 2^{x+y} \cdot 2^{a+b-y} \cdot n^{\calO(1)} =  
\sum_{\substack{a,b \\ x+a+b \leq k + 3}} 
 2^{x+a+b} 
 \cdot n^{\calO(1)} = 2^k \cdot n^{\calO(1)}
 $$
time to process all valid tuples in $\calV_k^{x, y}$. Since there are at most $\calO(k^2)$ feasible values for $x, y$, the overall running time of algorithm is bounded by $2^k \cdot n^{\calO(1)}$.
 This concludes the proof.
\end{proof}

